The information geometry of large language models is shared, learned, and controllable

Large language models learn similar behaviours, yet it remains unclear what structure they share or how to change one behaviour without disturbing others. The Fisher-Rao geometry of next-token probabilities connects these questions: behaviour determines this geometry up to output-preserving symmetries, whereas activation geometry depends on coordinates. Across transformer, state-space and recurrent models, output geometries agree more strongly than activation geometries, and shared geometry supports semantic-category transfer. Agreement with human word choices increases with predictive accuracy, scale and training, and improves further after model-only calibration. Token probabilities and read-out geometry jointly predict the spectrum and its effective dimension. Controlled language assignments show that geometry follows the language law across architectures. Pretraining corpus statistics predict held-out fact acquisition without recalibration, while randomised experiments show that deeper evidence substantially delays acquisition across every tested architecture and evidence construction. Finally, the geometry prescribes minimum-disturbance local interventions, predicts their relative cost, and supports reusable control: updates learned on donor prompts transfer to unseen prompts while better preserving behaviour on reference prompts than Euclidean control. The same geometric correction improves steering, editing, attribution, dictionary learning and fine-tuning.

==> references-main.tex <==
%
%
\makeatletter
\newlabel{Main-fig:ident}{{1}{3}{\textbf {Behaviour identifies the resolved read-out, and geometry predicts local output change.} \textbf {a}, Behavioural identification: held-out predictive loss after re-optimising nuisance parameters grows linearly with the squared subspace distance between a perturbed read-out subspace and the resolved subspace (Pythia 70M--1.4B). Markers are the 40 model--condition--angle means and bars span the two independently calibrated held-out folds (smaller than the markers); paths connect angles within each model and condition. Green, read-out deviation; grey, matched-random control; circles, 70M; squares, 160M; triangles, 410M; diamonds, 1.4B. The local fits have $R^2 \ge 0.9999$ on all eight paths, and matched-random control directions have systematically smaller loss--distance slopes (slope ratios $1.14$--$1.27$). The reference subspace is estimated from a stronger model (Supplementary Note~\ref *{SI-si:identification}). \textbf {b}, Predicted and measured output change under small activation perturbations. Each point is one model--depth--prompt combination, giving 99 measurements across 11 models, six families and quarter-, half- and three-quarter-depth injection. The prediction $\tfrac 12\delta h^\top G\delta h$ uses the metric before the intervention, without a fitted scale. Points show the coarsest resolved local steps; colour identifies the model and the grey line marks equality. The measured-to-predicted KL ratio has median $1.000$ and range $0.948$--$1.224$ (Methods; Supplementary Note~\ref *{SI-si:theory})}{figure.caption.3}{main.pdf}}
\newlabel{Main-eq:metric}{{1}{4}{Predictive behaviour fixes a canonical, identifiable output geometry}{equation.1}{main.pdf}}
\newlabel{Main-eq:ident}{{2}{4}{Predictive behaviour fixes a canonical, identifiable output geometry}{equation.2}{main.pdf}}
\newlabel{Main-eq:imprint}{{3}{6}{The geometry inherits the statistics of language}{equation.3}{main.pdf}}
\newlabel{Main-fig:shared}{{2}{7}{\textbf {Predictive geometry is shared across models and approaches human completion structure.} \textbf {a}, Output Fisher--Rao agreement against activation-space agreement on natural text for all 29 cross-tokenizer, cross-family dyads among ten models (70M--7B; transformer, state-space and recurrent). Each dyad contributes a blue mid-layer circle and vermilion last-layer square joined by a horizontal line; the grey line is equality. The output relation is stronger than either activation relation for every displayed mark. \textbf {b}, Absolute held-out error of the exchangeable six-scalar prediction across ten public training checkpoints. Circles show all 96 defined predictions; colours distinguish individual comparisons and lines follow them across training. Six predictions are defined per checkpoint at steps 1--64 and twelve from step 256; estimator definitions and early-checkpoint coverage are given in Supplementary Note~\ref *{SI-si:stabatten}. \textbf {c}, Native model samples approach human completions with scale. Points show all 96 context-fold means, 16 at each Pythia size; colours identify models in panels c and d. The ordinate is squared distance between semantic kernel means, cross-fitted over participant and model-sample halves (512 contexts, 32 samples per context; eight-token generation limit). No human-answer restriction is applied to sampling. \textbf {d}, A relation between conditional prediction risk and human semantic alignment fitted on Pythia is applied without refitting to five OLMo checkpoints and five external models. Points show all 160 model--context-fold comparisons; checkpoints and folds are repeated measurements. Alignment is reliability-corrected kernel CKA on a separate 384-context battery, using model laws conditional on the observed completion events. The grey line is equality; correlation $0.758$, root-mean-square error $0.0295$}{figure.caption.5}{main.pdf}}
\newlabel{Main-fig:imprint}{{3}{9}{\textbf {Language statistics shape the spectrum and its effective dimension.} \textbf {a}, Profile-predicted against measured spectral exponent over ranks 8--32 for all 576 held-out model--context cells (nine models from five external families, 64 contexts per model). Small circles show every cell and the grey line is exact prediction. Colours identify models throughout the figure. The Pearson and Spearman correlations are 0.968 and 0.955; family-median absolute exponent errors are $0.0623$--$0.0856$. On a matched 16-context-per-model control battery, spectral errors are $4.89$--$9.22$-fold lower than for a same-trace flat spectrum and $13.55$--$25.63$-fold lower than after shuffling profile ranks. \textbf {b}, Prediction of effective dimension without fitted parameters, the number of modes resolved at a given damping, from token statistics. Small circles show all 5,760 model--context--resolution values from the same 576 cells, coloured by model; the grey diagonal is exact prediction. No measured eigenvalue or fitted parameter enters the prediction. Family-median effective-dimension RMSEs are $0.0270$--$0.0521$, $6.44$--$7.88$-fold lower than for the same-trace flat-spectrum prediction. \textbf {c}, Effective-dimension prediction in a matched 14-model, seven-family comparison on 192 fresh contexts per model. All 2,688 points compare the weighted-profile and probability-only prediction errors on the same context, measured as effective-dimension RMSE across damping levels. The probability-only profile $\widehat \lambda _k=(r/V)p_{(k)}$ has lower family-median error in all seven families. \textbf {d}, All 672 paired spectral-exponent errors on the 48-context exact-spectrum subset per model; the weighted profile has lower family-median error in all seven families. Both panels use logarithmic axes, a common 27,450-outcome representation and the same standardised read-out; the grey diagonal marks equal error. Inference gives equal weight to families. Exact one-sided family sign-flip $P=1/128$ for each contrast (Supplementary Note~\ref *{SI-si:anatomy})}{figure.caption.7}{main.pdf}}
\newlabel{Main-fig:acq}{{4}{10}{\textbf {Corpus statistics predict acquisition across model sizes.} \textbf {a}, Ex-ante corpus n-gram margins predict subsequent margins without refitting for fresh facts disjoint from calibration at Pythia 70M, 160M and 410M. Points are all 9,840 fact--checkpoint means over 15 checkpoints: 5,340 from 178 defined facts at 70M and 160M (ten runs) and 4,500 from 300 facts at 410M (nine runs); the shared model-colour key below the panels distinguishes Pythia 70M, 160M and 410M; the grey diagonal is exact prediction. Trajectory $R^2$ is $0.790$, $0.792$ and $0.775$, persistent-status agreement is $0.792$, $0.854$ and $0.807$, and continuous timing error is $0.77$, $0.95$ and $0.96$ $\log _2$ training-step units, respectively. All three timing errors outperform their constant acquisition-time and label-permutation baselines. \textbf {b}, Cumulative acquisition curves for the same 300 facts against training step at 70M, 160M and 410M. Thin curves are individual seeds and heavy curves with circular markers are medians over nine seeds for each model size, using the shared model colours. \textbf {c}, The same curves against held-out loss. In the descriptive 70M-to-160M comparison, alignment by held-out loss has a median absolute error of 2.1 facts}{figure.caption.9}{main.pdf}}
\newlabel{Main-eq:control}{{4}{11}{The geometry determines minimum-disturbance interventions and their relative cost}{equation.4}{main.pdf}}
\newlabel{Main-fig:price}{{5}{12}{\textbf {The geometry predicts intervention cost and supports reusable control.} \textbf {a}, At matched behaviour change, the measured ratio of off-target output divergence for Euclidean versus damped natural-gradient updates is compared with the finite-damping prediction $R_{\mathrm {pred}}$, which has no fitted parameters and is computed before intervention. The axes are logarithmic and the grey identity line denotes perfect agreement. Small circles show all 3,515 usable matched-response observations (of 3,564) from 1,188 model--objective--layer--context cells: 11 models, six families, three objectives, three relative layer depths and 12 contexts per objective, each measured at three intervention magnitudes (98.6\% coverage; median measured-to-predicted ratio $0.967$, 95\% interval $0.957$--$0.975$; log--log slope $0.982$, 95\% interval $0.966$--$0.997$). \textbf {b}, Finite paths with both methods relinearised after every accepted step. All 864 points compare Euclidean and Fisher cumulative local KL at matched target changes, from 216 prompts, 16 models and 18 model--objective cells. The metric sums KL between successive accepted outputs. The 72 cell--target geometric-mean cost ratios span $11.5$--$127.1$, with every paired 95\% interval above one. Colours identify models in panels a and b. \textbf {c}, Reusable control on four base models from three families. All 192 points compare reference-Fisher sequence KL with Euclidean (vermilion) or donor-only Fisher (grey) sequence KL for the same reference continuation and matched donor change, across two objectives and three target changes. Each setting contributes four reference continuations per comparator. Reference sequences are teacher-forced continuations of the four prompts used to construct the reference metric. Ratios of mean Euclidean/reference-Fisher sequence KL span $2.90$--$6.29$. \textbf {d}, The same updates change unseen target prompts without target gradients. Each point shows mean sequence KL over four reference continuations and mean target log-odds change (nats) over eight unseen prompts, for one model, objective, donor change and method (48 points). Green, natural gradient using the reference metric; vermilion, Euclidean. Grey segments join matched donor changes. All 24 natural-gradient mean target changes are positive. Grey diagonals in panels b and c mark equality}{figure.caption.11}{main.pdf}}
\newlabel{Main-tab:operations}{{1}{14}{\textbf {One correction spans the evaluated operations.} The result column reports the strongest reported matched comparison for each operation; the final column gives its evidence base. Intervals are 95\% bootstrap intervals. AUC, area under the curve; KL, Kullback--Leibler; LoRA, low-rank adaptation. Sources and protocols are given in Methods}{table.caption.13}{main.pdf}}
\newlabel{Main-fig:ed-coordinate-controls}{{1}{32}{\textbf {Extended Data Fig.~\thefigure {} $|$ Coordinate covariance and common-outcome controls.} \textbf {a}, Coordinate covariance at finite damping. For 12 prompts under one seeded symmetric positive-definite gauge family with $\kappa (A)=1,3,10,30,100$, transporting the reference as $R'=A^{-\top }RA^{-1}$ reproduces the native damped direction with mapped relative error at most $7.4\times 10^{-13}$ (green circles). Installing a fresh identity instead changes the regularised problem: over non-identity gauges, the mapped-direction error has median 1.23 and minimum 0.54 (vermilion squares). Points, prompts; connected symbols, medians; error bars, 2.5th--97.5th percentiles. Pythia-410M, final pre-unembedding activation, top-512 output-Fisher support and $\alpha =0.01\lambda _{\max }$. \textbf {b}, Pairwise output-geometry agreement before and after mapping each next-token law to its first-byte distribution (21 dyads among eight models). Aggregate agreement is $0.899$ at token level and $0.910$ after the push-forward; rank agreement between dyad-level values is $0.551$. The grey line marks equality. \textbf {c}, Hidden-coordinate reparameterisation at nine anisotropy strengths and three seeds. Each point aggregates the same 21 model pairs; faint paths show seeds and heavy paths their means. Output Fisher--Rao agreement remains constant, while activation CKA, mutual nearest-neighbour overlap and cosine RSA degrade. Small horizontal offsets separate seeds}{figure.caption.70}{main.pdf}}
\newlabel{Main-fig:ed-displacement-null}{{2}{33}{\textbf {Extended Data Fig.~\thefigure {} $|$ Shared output structure beyond displacement magnitude and on independent human data.} \textbf {a}, The 24 displayed estimates are six fixed eigenvalue-rank bands crossed with four summaries: raw subspace overlap (grey circles), a displacement-magnitude-matched null that preserves each word's displacement magnitude (amber squares), a shuffled-word null (magenta triangles) and the residual above the displacement-magnitude-matched null (blue diamonds). Opaque markers have black borders; lines connect like summaries across bands. Error bars on the residual span the 2.5th--97.5th percentiles across 400 random 80\%-context subsamples. Raw overlap is nearly flat, but the residual is concentrated in the leading modes and falls from $0.080$ in ranks 0--5 to $0.013$ in ranks 90--120. Thus about 89\% of the leading-band raw overlap is explained by shared displacement magnitudes, while the smaller residual carries the rank-dependent cross-family structure. \textbf {b}, Native model samples on 640 word positions from five previously unused narratives. Points are the equal-story semantic distances for six final Pythia sizes; bars show conditional 95\% bootstrap intervals and the grey line is the registered fit against log parameter count (slope $-0.00872$, interval $-0.01202$ to $-0.00556$). \textbf {c}, The same distance at five ordered checkpoints from Pythia-160M and OLMo-2-1B. Lines show point estimates and shaded regions the conditional 95\% intervals. Final-minus-initial changes are $-0.12080$ and $-0.10962$, respectively. \textbf {d}, Expected human log-score change after applying the model-only source-trained full 65-outcome map instead of each model's native law. Small circles show the five fixed-story differences and diamonds their equal-story means; positive values favour calibration. Six of seven family means are positive ($0.0196$--$0.0507$ nats); Qwen2 is $-0.0030$ nats. Panels b--d are conditional on the five observed stories and make no population-of-stories claim}{figure.caption.71}{main.pdf}}
\newlabel{Main-fig:ed-effective-dimension}{{3}{34}{\textbf {Extended Data Fig.~\thefigure {} $|$ Damping reveals bounded effective dimension.} \textbf {a}, Predicted versus measured stiff-mode counts for 24 model--context spectra at relative damping $10^{-1}$, $10^{-2}$ and $10^{-3}$ (72 points). Predictions are $(1/c)^{1/\beta }$ from the power-law exponent fitted over ranks 2--80; colours identify the eight models, and the grey line denotes equality. \textbf {b}, All 72 resolved-mode counts, joined within each of the 24 spectra; colours identify models and black diamonds show the cross-spectrum median. The count grows as damping is lowered. The native-reference exponent is empirically stable across the tested models but is not an invariant of the metric alone. In held-out estimator validation, nominal 95\% interval coverage is $0.90$ for continuous effective dimensions and $0.85$ for discrete threshold counts; primary dimension estimates therefore use the continuous form (Methods). \textbf {c}, Finite-size effective-dimension confirmation on 80 model--prompt curves spanning ten models and seven families. For each curve, a bounded effective-dimension curve was fitted at four fixed anchor dampings; points are all 240 observations at three interleaved, held-out dampings after rescaling by the fitted crossover $\alpha ^{*}$. The black line is the bounded effective-dimension curve at the median fitted exponent. \textbf {d}, Curve-level held-out root-mean-square error for an equal-parameter unbroken power law (abscissa) and the bounded effective-dimension curve (ordinate). Every one of 80 points lies below equality. Median errors are $0.0814$ and $0.00493$, respectively; the median bounded-to-power error ratio is $0.0749$ (95\% crossed-bootstrap interval $0.0428$--$0.1234$)}{figure.caption.72}{main.pdf}}
\newlabel{Main-fig:ed-acq-generalisation}{{4}{35}{\textbf {Extended Data Fig.~\thefigure {} $|$ Evidence depth delays acquisition across architectures and evidence constructions.} \textbf {a}, Randomised evidence depth delays persistent acquisition. Curves follow the 10th--20th acquisition-time percentiles for each of 12 training seeds of the same transformer, pooling over the same facts and probes within each seed. Black curves show individual seeds; blue, pink and green shading to their right marks acquisition levels already reached under shallow, intermediate and deep evidence, respectively. The pooled deepest-versus-shallowest shift is $\Delta =2.10$ $\log _2$ training-step units (crossed seed-by-quintet bootstrap 95\% interval $1.79$--$2.40$), equivalent to $4.3\times $ more training steps; the deepest-versus-intermediate contrast is smaller. \textbf {b}, Mean paired delay in persistent acquisition for evidence assigned to the deep construction relative to otherwise matched evidence in the shallow construction, crossing GPT-2-, GPT-NeoX- and Llama-style decoders with copy-back-reference and four-cue-parity controlled languages. Blue diamonds denote copy-back-reference cells and amber diamonds four-cue-parity cells; horizontal lines are 95\% crossed seed-by-matched-block bootstrap intervals around the cell means over eight seeds and 384 matched fact blocks per cell. All six intervals and all 48 seed means are positive; effects span $0.810$--$1.514$ $\log _2$ training-step units ($1.75$--$2.86$-fold in training steps). The equal-family mean parity-minus-back-reference contrast is $0.414$ $\log _2$ training-step units (95\% interval $0.291$--$0.536$). \textbf {c}, Corresponding fixed-treatment (blue circles) and label-randomisation (vermilion squares) controls. Every one of the twelve 95\% intervals contains zero. The grey vertical line in panel c marks zero delay; delays are in $\log _2$ training-step units}{figure.caption.73}{main.pdf}}
\newlabel{Main-fig:ed-intervention-frontiers}{{5}{36}{\textbf {Extended Data Fig.~\thefigure {} $|$ Additional intervention trade-off curves, composition and fixed activation editing.} \textbf {a}, The diffuse style objective: behaviour change against off-target change on neutral prompts. The complete 19-point operating sweep contains seven Fisher, six Euclidean and six contrastive-activation-addition (CAA) settings. \textbf {b}, Composition: sycophancy and style steered simultaneously by one solve on the weighted covector sum; varying the weight changes the balance between objectives, whereas summed CAA vectors change sycophancy in the opposite direction. The 20 distinct operating points produce 34 displayed objective outcomes; all markers are opaque with black borders. \textbf {c}, Matched fixed activation edits on 30 held-out CounterFact records (GPT-2). Each point compares Fisher other-token Kullback--Leibler (KL) divergence (abscissa) with Euclidean other-token KL divergence (ordinate) after both operators attained the same fixed $+5$ log-odds shift; axes are logarithmic and the grey line denotes equality. Euclidean cost is higher for all 30 edits, with a geometric-mean Euclidean-to-Fisher ratio of $10.57$ (95\% interval $8.52$--$13.37$)}{figure.caption.74}{main.pdf}}
\newlabel{Main-fig:ed-feature-selectivity}{{6}{37}{\textbf {Extended Data Fig.~\thefigure {} $|$ Output geometry predicts the causal cost and selectivity of sparse features.} Pythia-410M, layer 12, Top-$k$ sparse autoencoder. Points in every panel are the same 303 unique zero ablations of active sparse-autoencoder (SAE) features from 57 evaluation-active features across 18 held-out context clusters; feature and objective selection used 18 disjoint discovery contexts. Opaque green points in \textbf {a} and \textbf {c} mark Fisher quantities, while blue points in \textbf {b} mark attribution patching; every point has a black border. \textbf {a}, The Fisher prediction $\tfrac 12\Delta h^\top G\Delta h$ against exact full-vocabulary $\mathrm {KL}(p_0\Vert p_{\mathrm {zero}})$ (Spearman $\rho =0.997$); grey line, equality. \textbf {b}, Attribution-patching magnitude against the selected-token probability-change fraction, the fraction of full-vocabulary absolute probability change on discovery-selected tokens ($\rho =0.506$). \textbf {c}, The objective-effect-to-Fisher-cost ratio against the same endpoint ($\rho =0.935$); its correlation exceeds that of attribution patching by $0.429$ (95\% context-cluster bootstrap interval $0.296$--$0.553$). The comparison concerns concentration on selected tokens; attribution-patching magnitude remains the stronger predictor of absolute effect magnitude}{figure.caption.75}{main.pdf}}
\newlabel{Main-fig:ed-lora-preservation}{{7}{38}{\textbf {Extended Data Fig.~\thefigure {} $|$ Natural-gradient low-rank adaptation lowers held-out preservation cost at matched training gain.} Exact natural-gradient LoRA is compared with tuned AdamW with explicit KL regularisation using rank-4 adapters on Pythia-70M. Points are all 48 method--target--seed cells from eight paired outer seeds, three fixed matched training-gain targets and two methods; each cell averages 16 held-out preservation prompts. Vermilion squares denote AdamW+KL and green circles exact natural gradient. Pale lines join paired methods within seed and target, horizontal offsets are fixed display jitter, and the larger connected symbols are method means. The ordinate is logarithmic. Every method reached every target. Across this frontier, AdamW+KL incurred $1.57\times $ the preservation-KL AUC of exact natural gradient (95\% paired hierarchical bootstrap interval $1.14$--$1.98$). The experiment did not support a broader task-transfer or capability-retention conclusion}{figure.caption.76}{main.pdf}}
\newlabel{Main-fig:ed-layer-magnitude}{{8}{38}{\textbf {Extended Data Fig.~\thefigure {} $|$ Layer and intervention magnitude delimit the geometric correction.} \textbf {a}, Off-target advantage by injection layer for 3,515 usable matched-response observations from 1,188 model--layer--objective--context cells across 11 models and six families, summarized as 33 within-model estimates. Coloured circles are geometric means and vertical bars are 95\% paired objective--context--magnitude bootstrap intervals that preserve the available layer tuple; lines connect the three depths within model. Black diamonds are model-balanced geometric means with 95\% model-bootstrap intervals. The pooled means fall from $11.79$ to $11.08$ to $6.62$ at quarter, half and three-quarter depth, respectively. Every model mean is lower at three-quarter than at quarter depth; nine of eleven paths decrease at both adjacent steps, with one intermediate-depth increase for Mamba 130M and Qwen2 1.5B. \textbf {b}, Measured-to-predicted off-target advantage at intervention fractions $\Delta C/C=0.01,0.03,0.10$. Coloured circles are all 33 within-model geometric means (11 models crossed with three fractions), with 95\% paired-cell bootstrap intervals; lines connect fractions within model. Black diamonds are model-balanced geometric means with model-bootstrap intervals, and the grey line denotes exact calibration. All 11 model paths decrease strictly. The model-balanced means are $0.918$, $0.860$ and $0.755$, quantifying the expected attenuation of a local prediction as intervention magnitude grows}{figure.caption.77}{main.pdf}}
\newlabel{Main-fig:ed-colocalisation}{{9}{39}{\textbf {Extended Data Fig.~\thefigure {} $|$ Output sensitivity, cross-model sharing and answer motion concentrate in the same native-reference modes.} Each panel shows all 21 summaries (seven predefined eigenvalue-rank bands $\times $ three quantities) from six models: the band's eigenvalue-mass share, cross-model eigenvector sharing against the displacement-magnitude-matched null and probability motion on the highest-probability tokens. To compare their decay directly, each quantity and its 95\% context-bootstrap interval are divided by that quantity's leading-band point estimate. On natural text the top five modes carry 55\% of the eigenvalue mass, the largest residual sharing ($+0.069$, 95\% interval $0.062$--$0.077$) and the largest answer motion ($0.59$), all three decaying together to the last band. \textbf {a}, Natural-text battery. \textbf {b}, Templated battery}{figure.caption.78}{main.pdf}}
\newlabel{Main-fig:cyclic}{{10}{40}{\textbf {Extended Data Fig.~\thefigure {} $|$ Two geometries of behaviour: cyclic reweighting and relation-induced probability displacement} (Pythia-410M). \textbf {a},\textbf {b}, Walking the ring by steering month$\to $month (\textbf {a}) or day$\to $day (\textbf {b}) around the full cycle at matched concept progress: the plane is the concept's phase circle in output space and height is accumulated off-target change (bits). Both paths traverse the same ordered concept cycle; the reference phase sectors are separated, by construction, by $2\pi /12$ (or $2\pi /7$). After one circuit the endpoint returns towards the starting sector with a method-dependent residual displacement, while the natural-gradient path accumulates less off-target change. \textbf {c}, The dissociation from analogy relations. Paired circles and squares show probability-displacement alignment and its permuted control for all twelve concept sets across three categories (24 displayed values); thin grey lines join each concept's pair and short horizontal bars show category means. Relations move mass along a shared probability-displacement direction (mean alignment $0.49$; permuted control $0.33$), while cyclic concepts show none ($0.00$) and are near-isometries of the metric. The shared colour key applies to both trajectory panels}{figure.caption.80}{main.pdf}}
\makeatother

